Helly theorem for affine spaces without dimensions

We prove a no-dimensional Helly theorem for affine spaces and convex sets using the unboundedness framework of Aronov, Goodman, and Pollack (Computational Geometry, 2002). This generalizes the fundamental result of Adiprasito, B\'ar\'any, Mustafa, and Terpai on the no-dimensional Helly theorem for points and convex sets (Discrete & Computational Geometry, 2020). Additionally, we establish the optimality of our result.

==> abstract.tex <==


\begin{abstract}
    We generalize the no-dimensional Helly Theorem for points by Adiprasito, B\'{a}r\'{a}ny, Mustafa, and Terpai ({\em Discrete \& Computational Geometry} 2020) to $k$-flats (affine subspace of dimension $k$). 
    Using the $k$-unbounded framework of Aronov, Goodman and Pollack ({\em Computational Geometry} 2002) we prove a no-dimensional colorful Helly Theorem for $k$-flats for families of closed convex sets in $\R^{d}$. 
    We complement the above result with a number of impossibility results establishing the optimality of our extension.
\end{abstract}













==> intro.tex <==
\section{Introduction}



Helly Theorem is a fundamental result in discrete and convex geometry. The theorem states that given any finite collection $\F$ of convex sets in $\R^d$, if the sets in every subfamily of $\F$ of size $d+1$ have a point in common, then all the sets in the entire family $\F$ have a point in common. Note that the finiteness of $\F$ can be relaxed if we assume that the convex sets in $\F$ are compact, therefore unless otherwise stated explicitly, we will not assume anything about the cardinality of a collection.
Since its discovery~\cite{Helly23}, Helly Theorem has found multiple applications and generalizations~\cite{Eckhoff1993helly,AmentaLP2017,DeLoeraGMM2019discrete,BaranyK2022helly}.


We say a set $T \subseteq \R^{d}$ {\em pierces} a family $\F$ of subsets of $\R^{d}$ if all sets in $\F$, has a non-empty intersection with the set $T$.  
A natural generalization of Helly Theorem would be to consider the problem of piercing a family of convex sets with a $k$-flats\footnote{By $k$-flat we mean affine subspace of $\R^{d}$ of dimension $k$. Note that by lines and hyperplanes, we will mean $1$-flats and $(d-1)$-flats respectively.}.
Results of the above form are called {\em Helly-type} results. 
Generally, we want to show that there exists an integer $h(k,d)$ such that if any $h(k,d)$ convex sets from a collection $\F$ can be pierced by a $k$-flat then the whole collection $\F$ can be pierced by a $k$-flat. Unfortunately, Santal\'{o}~\cite{Santal2009} showed the impossibility of getting such a result for even piercing a collection of convex sets by a line.  
Hadwiger~\cite{Hadwiger56} showed that for a countable collection $\F$ of disjoint convex sets in $\R^{d}$ with non-empty interior and all congruent to a fixed compact convex set $C$, if every $d+1$ sets from $\F$ can be pierced by a line then the whole family can be pierced by a line. 
Later, 
Danzer, Gr\"unbaum and Klee~\cite{DGK} showed that the "congruent" assumption in Hadwiger's result~\cite{Hadwiger56} can be weakened if the convex sets have bounded diameters. 
Aronov, Goodman, Pollack, and Wenger~\cite{ABJP} proved the first Helly-type result for hyperplanes about families of {\em well-separated} compact convex sets of arbitrary shapes in higher dimensions. 
Later, 
Aronov, Goodman, and Pollack~\cite{AronovGP2002} showed a Helly-type result for $k$-flat for families of convex bodies that are {\em unbounded} in $k$-independent directions.



Adiprasito, B\'{a}r\'{a}ny, Mustafa, and Terpai~\cite{AdiprasitoBMT2020} in a breakthrough paper proved the first no-dimensional variant of the classical Helly Theorem:
\begin{theorem}[Adiprasito, B\'{a}r\'{a}ny, Mustafa, and Terpai~\cite{AdiprasitoBMT2020}]\label{Point}
	Let $C_{1},\dots,C_{n}$ be convex sets in $\R^d$ and $r \in \left\{ 1, \dots, n\right\}$. 
	For $J \subseteq \left\{ 1, \dots, n \right\}$, let $\mathcal{C}(J)\coloneqq \bigcap_{j\in J} C_j$. 
	If $B(b,1)$ intersects $\mathcal{C}(J)$ for every $J \subseteq \left\{ 1, \dots, n \right\}$ 
    with $|J| = r$, then there is a point $q\in\R^d$ such that for all $i \in \left\{1, \dots, n \right\}$ we have
	\begin{equation}
		d(q,C_i)\leq \sqrt{\frac{n-r}{r(n-1)}}
        \; .
	\end{equation}
    Observe that for a fixed $k$ and $n\to\infty$, the right-hand side of the above equation approaches $\frac{1}{\sqrt{r}}$. 
 
    Note that for all $q \in \R^{d}$ and $S \subseteq \R^{d}$, $d(q,S)$ denotes the distance between the point $q$ and the set $S$, that is, $$
        d(q,S) := \inf_{x \in S} \|q-x\|.
    $$
    Also, note that $B(x,R)$ denotes a closed Euclidean ball centered at $x \in \R^{d}$ with radius $R$.
\end{theorem}
They also proved the following colorful variant of the above theorem. 
\begin{theorem}[Adiprasito, B\'{a}r\'{a}ny, Mustafa, and Terpai~\cite{AdiprasitoBMT2020}]\label{PointColor}
	Let $\F_{1}, \dots, \F_{r}$ be families of convex sets in $\R^d$ with $r\leq d$, and 
    $b \in \R^{d}$. 
	Assume that for any $r$-tuple $\left(C_{1}, \dots,C_{r}\right)$ with $C_i\in\F_i$ for all $i \in \left\{1, \dots, r \right\}$, we have 
    $$
        \left(\bigcap_{1 \leq i \leq r }C_{i}\right) \bigcap B(b,1) \neq \emptyset.
    $$
    Then there exists a point $q\in\R^d$ and  $\exists i \in \left\{ 1, \dots, r\right\}$ such that $\forall C\in\cF_i$ we have $d(q,C)\leq \dfrac{1}{\sqrt{r}}$.
%	\begin{equation}
%		d(q,C)\leq \frac{1}{\sqrt{r}}.
%	\end{equation}
\end{theorem}
We generalize the above results for points to $k$-flats. We also prove some impossibility results which establish the optimality of our generalization. 


\paragraph{Notations.}
Throughout the rest of the paper we use the following notations:
\begin{itemize}
    \item 
        Origin of $\R^{d}$ will be denoted by $\mathcal{O}$.

        
    \item 
        For all $n \in \N$, $[n]$ denotes the set $\left\{ 1, \dots, n\right\}$.
    
    \item 
        For any two points $p$ and $q$ in $\R^{d}$, the Euclidean distance between $p$ and $q$ will be denoted by $\|p-q\|$.

    \item 
        $|X|$ will denote the size of a set $X$.
    
    \item
        The diameter of the set $C \subseteq \R^{d}$ will be denoted by $\text{diam}(C)$.
    
    \item 
        For all $b \in \R^{d}$ and $r > 0$, {\em closed} and {\em open balls} centered at the point 
        $b$ and radius $r$ will be denoted by  
        $$
            B(b,r) : = \left\{p \in \R^{d} \, : \, \|p-b\| \leq r \right\}
        $$ 
        and
        $$
            B^{o}(b,r) : = \left\{p \in \R^{d} \, : \, \|p-b\| < r \right\}
        $$
        respectively.

    \item   
        By $\mathbb{S}^{d-1}$ we will denote the $(d-1)$-dimensional unit sphere
        centered at the origin. 
    
    \item 
        The {\em distance} $d(S_{1}, S_{2})$ between two subsets $S_{1}$ and $S_{2}$ of $\R^{d}$ is defined as 
        $$
            d(S_{1}, S_{2}) : = \inf_{(p_{1}, p_{2}) \in S_{1}\times S_{2}} \|p_{1} - p_{2}\|.
        $$

    \item 
        Given points $p$ and $q$ in $\R^{d}$, $\overline{pq}$ denotes the closed line segment connecting $p$ and $q$.

\end{itemize}


==> justification.tex <==
\textbf{Proof of Theorem~\ref{impossibility}:}
\subsection{Compactness}

The necessity of the condition compactness in Theorems 
\ref{noDimKflat} and ~\ref{colorNoDimKflat} can be justified as follows.

Consider the set $\F$ of all half-planes not containing the origin generated by tangents to the circle centered at the origin with radius $2$ in $\R^2$.
Now for any $r$ half-planes in $\F$, we can find a straight line that intersects those half-planes and also passes through the origin.
But, there is no straight line that lies at a distance $1$ from all half-planes in $\F$, due to the fact that for every straight line $l$, there are two half-planes defined by straight lines parallel to $l$ and a distance $4$ apart from each other. Therefore, compactness is a necessary condition.

\subsection{$k$-unboundedness}

We choose the same set as in Aronov et al. \cite{AronovGP2002} to demonstrate that the $k$-unboundedness condition is necessary.

\begin{figure}[htpb]
    \centering
    \begin{tikzpicture}
        \draw (0,0) node{\includegraphics[scale=1]{kUGimp}};
    \end{tikzpicture}
    \caption{An example demonstrating the necessity of  
 $k$-unboundedness condition}
    \label{fig:k1}
\end{figure}

Consider Figure \ref{fig:k1}, that consists of a set of covex shaded regions created by four circles and four squares centered at a point $O$. Let the 
plane on which the shaded regions of Figure \ref{fig:k1} lie   be the $xy$-plane, and the point $O$ be the origin. Let these $8$ shaded regions be 8 sets, namely $a_1$, $a_2$, $\dots$, $a_8$, respectively.
Clearly, any $3$ of these regions can be intersected by a straight line. We now create additional sets as follows by repeating the following process.

In each step, we enlarge the $8$ sets, obtained in the last step, slightly so that they remain pairwise disjoint, and then we elevate those sets, one at a time in a chosen order in rapidly increasing heights (to be described later) along the $z$-axis. This gives us a countably infinite sequence $\F$ of sets, where $\F$ is $1$-unbounded, but not $2$-unbounded.
It is shown in Aronov et al.\cite{AronovGP2002} that for any $4$ sets in $\F$, there exists a plane that passes through $O$ and intersects these $4$ sets, provided the sets were elevated appropriately. 

Let $\ell$ denote the length of the side of the smallest square in Figure \ref{fig:k1}.
We show that it is not possible to find a plane that is at most a distance 1 unit away from all the sets in $\F$ when $\ell$ is large enough.
Let, if possible, $K$ be such a plane.
Clearly, $K$ must be perpendicular to the plane that contains the first $8$ sets. 
By symmetry, we can take $K$ to be passing through $O$.
Let $T$ be the intersection of $K$ and the $xy$-plane, and let the side-lengths of the $4$ squares in Figure \ref{fig:k1} be $l_1 (=\ell), l_3, l_5, l_7$, where the side of side-length $l_i$ is shared by the set $a_i$.
Let the diagonals of the largest square in Figure \ref{fig:k1} lie on the $x$-axis and the $y$-axis respectively.
Then, if $T$ makes an angle $\theta\in[0,\pi)$ with the $x$-axis, then we have the following:
\begin{itemize}
    \item For $i=1,3,5,7$, $d(T,a_i)=d(T,a_{i+1})$, and 
    \item 
        \begin{equation}
            d(a_1,T)=
            \begin{cases}
                \frac{l_1}{\sqrt{2}}\sin(\frac{\pi}{4}-\theta) & \text{if } 0\leq\theta\leq\frac{\pi}{4}\\
                \frac{l_1}{\sqrt{2}}sin(\pi-\theta) & \text{if } \frac{3\pi}{4}\leq\theta\leq\pi\\
                0 & \text{otherwise}
            \end{cases}
        \end{equation}
    \item 
        \begin{equation}
            d(a_3,T)=
            \begin{cases}
                \frac{l_3}{\sqrt{2}}\sin\theta & \text{if } 0\leq\theta\leq\frac{\pi}{4}\\
                \frac{l_3}{\sqrt{2}}\sin(\frac{\pi}{2}-\theta) & \text{if } \frac{\pi}{4}\leq\theta\leq\frac{\pi}{2}\\
                0 & \text{otherwise}
            \end{cases}
        \end{equation}
    \item 
        \begin{equation}
            d(a_5,T)=
            \begin{cases}
                \frac{l_5}{\sqrt{2}}\sin(\theta-\frac{\pi}{4}) & \text{if } \frac{\pi}{4}\leq\theta\leq\frac{\pi}{2}\\
                \frac{l_5}{\sqrt{2}}\sin(\frac{3\pi}{4}-\theta) & \text{if } \frac{\pi}{2}\leq\theta\leq\frac{3\pi}{4}\\
                0 & \text{otherwise}
            \end{cases}
        \end{equation}
    \item 
        \begin{equation}
            d(a_7,T)=
            \begin{cases}
                \frac{l_7}{\sqrt{2}}\sin(\theta-\frac{\pi}{2}) & \text{if } \frac{\pi}{2}\leq\theta\leq\frac{3\pi}{4}\\
                \frac{l_7}{\sqrt{2}}\sin(\pi-\theta) & \text{if } \frac{3\pi}{4}\leq\theta\leq\pi\\
                0 & \text{otherwise}
            \end{cases}
        \end{equation}
\end{itemize}

\noindent Clearly, $\sum_{i=1}^{8} d(T,a_i) \ge \frac{\ell}{\sqrt{2}}\min_{\theta\in[0,\frac{\pi}{4}]}(\sin\theta+\sin(\frac{\pi}{4}-\theta))\ge \ell\sqrt{2}\sin\frac{\pi}{8}$.
Thus, for $\ell>\sqrt{2}/\sin\frac{\pi}{8}$, there are no planes that are at most $1$ distance away from each set in $\F$.

\subsection{Tightness of the bound}
\noindent We provide an example where the bound given in Theorem \ref{colorNoDimKflat} is tight.

\begin{figure}[htpb]
    \centering
    \begin{tikzpicture}
        \draw (0,0) node{\includegraphics[scale=1.2]{Bound}};
    \end{tikzpicture}
    \caption{}
    \label{fig:bound2}
\end{figure}
\noindent Let $ABCDEFGH$ be a cube in $\R^3$ such that its centroid is the origin $O$ and $EFGH$ lies on a plane parallel to the $xy$-plane (see Figure \ref{fig:bound2}) and each of its sides has length $\sqrt{2}$.
Define $\F_i\coloneqq\{S_{i,1},S_{i,2},S_{i,3},\dots\}$ for $i=1,2,3$ in the following way:
Set $S_{1,1}=\ol{AB}$, $S_{1,2}=\ol{CD}$ and $S_{1,n}$ is the line segment $\ol{CD}$ raised to the height $z=n$ for $n>2$.
Similarly, set $S_{2,1}=\ol{GH}$, $S_{1,2}=\ol{EF}$ and $S_{2,n}$ is the line segment $\ol{EF}$ lowered to the height $z=-n$ for $n>2$.
Now set $S_{3,1}=\ol{BC},S_{3,2}=\ol{DA},S_{3,3}=\ol{FG},S_{3,4}=\ol{HE}$, and let $S_{2,4n+j}$ be the set $S_{2,j}$, for all $j \in \{1,2,3,4\}$ (see Figure \ref{fig:bound2}).
Clearly, any colorful $3$-tuple $(C_1,C_2,C_3)$, $C_i\in\F_i$, $i\in[3]$, can be hit by a straight line that is at most at a distance $1$ away from the centroid.
Let $\mathcal{L}$ denote the set of all straight line transversals $l$ of colorful $3$-tuples such that $l$ is as close to $O$ as possible.
Let $l_n$ denote the straight line transversal in $\mathcal{L}$ that passes through $S_{1,n},S_{2,1},S_{3,1}$.
Clearly, $d(l_n,O)\to 1$ as $n\to\infty$.
Then, $\sup_{l\in\mathcal{L}}d(O,l)=1$.
Now note that for the straight line $L$ that is perpendicular to the plane on which $ABCD$ lies and passes through $O$, we have $\inf_{i\in[3]}\sup_{C\in\F_i}d(l,C)\ge\inf_{i\in[3]}\sup_{C\in\F_i}d(L,C)$ for any straight line $l$ in $\R^3$.
This we can show in the following way: let $l_1$ be a straight line such that $\sup_{C\in\F_1}d(l_1,C)=\inf_{l\in\mathcal{L}}\sup_{C\in\F_1}d(C,l)$.
Then $l_1$ must be perpendicular to the plane on which $ABCD$ lies, because otherwise the supremum of its distances from sets in $\F_1$ would be infinity.
Then, $l_1$ must be equidistant from both $S_{1,1}$ and $S_{1,2}$, and therefore, we can take $l_1$ to be $L$.
Similar arguments show that $\sup_{C\in\F_2}d(L,C)=\inf_{l\in\mathcal{L}}\sup_{C\in\F_1}d(C,l)$
We have $\inf_{i\in[3]}\sup_{C\in\F_i}d(L,C)=\frac{1}{\sqrt{2}}$.
To see that $\inf_{l\in\mathcal{L}}\sup_{C\in\F_3}d(C,l)=\frac{1}{\sqrt{2}}$, project $\ol{BC}$, $\ol{AD}$, $\ol{FG}$, $\ol{EH}$ onto the plane $P$ that contains $ABEF$.
If there is a straight line $l_3$ such that $\sup_{C\in\F_3}d(l_3,C)=\inf_{l\in\mathcal{L}}\sup_{C\in\F_3}d(C,l)$, then let the projection of $l_3$ onto $P$ be $l'_3$.
If $L$ is not the straight line that minimizes $\inf_{l\in\mathcal{L}}\sup_{C\in\F_6}d(C,l)$, then the perpendicular distance from $l'_3$ to $A,B,E$ and $F$ must be smaller than $\frac{1}{\sqrt{2}}$.
Let, without loss of generality, $A$ be the point from which $l'_3$ is the farthest.
Then, we must have another point among $B,E$ and $F$ from which $l'_3$ has the same distance as $A$.
This point then must be $E$, because otherwise we could have taken $L$ to be $l_3$.
This means that $l'_3$ passes through the centroid of the square $ABEF$ and two points from $A,B,E$ and $F$ lie on each side of $l'_3$.
But this implies that $l'_3$ must be parallel to $AB$ since $l'_3$ has the minimum distance from both $A$ and $B$ and is at least as close to $E$ and $F$, which is a contradiction.
We have $\inf_{i\in[3]}\sup_{C\in\F_i}d(L,C)=\frac{1}{\sqrt{2}}$, which is what we get by plugging in the values of $r$ and $k$ in the inequality given in Theorem \ref{colorNoDimKflat}.


==> notations.tex <==
\section{Our results}\label{defth}


Before we can give the statements of our results we need to first introduce some definitions which will be required to state our results. 
We define the {\em central projection map} $f:\R^{d} \to \mathbb{S}^{d-1}$, where $\mathbb{S}^{d-1}$ is the unit sphere centered at $O$, in the following way: for all $x \in \R^{d}$
$$
    f(x) : = \frac{x}{\|x\|}.
$$
We say $y \in \mathbb{S}^{d-1}$ is a {\em limiting direction} of the collection $\F$ if there exists a infinite sequence of points $\left\{ s_{n}\right\}_{n \in \mathbb{N}}$ and infinite sequence of sets $\left\{ S_{n}\right\}_{n \in \N}$ satisfying the following properties:
\begin{itemize}
    \item 
        for all $n \in \N$, $S_{n} \in \F$

    \item 
%       \color{red} 
       for all $n \neq m$ in $\N$, $S_{n} \neq S_{m}$ - 
       
%       \color{blue} Is this condition necessary? I think we should remove this \color{black}
    
    \item 
        for all $n \in \N$, $s_{n} \in S_{n}$
        
    \item
        $\lim\limits_{n \to \infty} \|s_{n}\| = \infty$ and 
        $\lim\limits_{n \to \infty} f(s_{n}) = y$
\end{itemize}
\noindent
For a collection $\F$ of subsets of $\R^{d}$, {\em limiting direction set} $LDS(\F)$ of $\F$ is defined as 
$$
    LDS(\F) : = \left\{ y \in \mathbb{S}^{d-1} \, : \, y\; \mbox{is a limiting direction of} \; \F \right\}.
$$
We will call the collection $\F$ {\em $k$-unbounded} if the vector space spanned by set $LDS(\F)$ has dimension at least $k$. Note that $k$-unbounded definition was first introduced by Aronov, Goodman and Pollack~\cite{AronovGP2002}. 
We prove the following {\em colorful} Helly Theorem for $k$-flats using the $k$-unbounded framework.



%Aronov, Goodman and Pollack~\cite{AronovGP2002} proved the following Helly-type theorem for $k$-flats:
%\begin{theorem}[Aronov, Goodman and Pollack~\cite{AronovGP2002}]\label{kflat}
%	Let $\F$ be a family of compact convex sets in $\R^d$ such that there exists an $R\in\R^{+}$ for which $diam(C)<R$ $\forall C\in\F$ and $\cup_{C\in\F}C$ is unbounded. Now, 
%$\F$ is $k$-unbounded if the limiting direction set of $\F$ has dimension greater than or equal to $k$. In addition, 
%if $\F$ is $k$-unbounded and any $d+1$ sets in $\F$ can be intersected by a $k$-flat, then there exists a $k$-flat that intersects all sets in $\F$.
%\end{theorem}

%One can prove a {\em colorful version} of the above theorem.

\begin{theorem}
    [Colorful Helly Theorem for $k$-flats]
    \label{col_aronov1}
    Suppose for each $i\in[d+1], \cS_i$ is a $k$-unbounded collection of compact convex sets in $\R^{d}$, and there exists $R > 0$ such that $\forall C \in \cS_{1} \cup \dots \cup \cS_{d+1}$ we have $\diam(C) < R$. 
    Also, assume that for every $(d+1)$-tuple $(C_{1}, \dots, C_{d+1}) \in \cS_{1}\times \dots \times \cS_{d+1}$ there exists a $k$-flat $H$ such that $H$ intersects $C_{i}$ for all $i \in [d+1]$. Then $\exists j\in[d+1]$ and a $k$-flat $\widetilde{H}$ that intersects every sets in $\cS_{j}$.
\end{theorem}
\noindent
Note that the above result is a colorful generalization of the Helly Theorem for $k$-flats proved by Aronov, Goodman and Pollack~\cite{AronovGP2002}
The following theorem is the main technical result in this paper, and we show that the rest of the results are a direct consequence of this result. 

\begin{theorem}[Colorful No-Dimensional Helly Theorem for $k$-flats]
    \label{main-result}
    Let $\F_{1}, \dots, \F_{r}$ be families of convex sets in $\R^{d}$, $k < r \leq d$, and the family $\F:= \F_{1} \cup \dots \cup \F_{r}$ of convex sets satisfy the following properties:
    \begin{description}
        \item[(i)] 
            $\exists R > 0$ such that for all $C \in \F$ we have $\diam(C) < R$

        \item[(ii)]
            $\exists J_{k} = \{ j_{1}, \dots, j_{k}\} \subset [r]$ and $\left\{ y_{j_{1}}, \dots, y_{j_{k}}\right\} \subset \mathbb{S}^{d-1}$ such that 
            \begin{itemize}
                \item 
                    for all $i \in J_{k}$ we have $y_{i} \in LDS\left( \F_{i} \right)$, and 
                \item 
                    the collection of vectors $\left\{ y_{j_{1}}, \dots, y_{j_{k}}\right\}$ are linearly independent 
            \end{itemize}
    \end{description}
    If for any $r$-tuple $\left(C_{1}, \dots, C_{r}\right) \in \F_{1}\times \dots \times \F_{r}$ there exists a $k$-flat that intersects the closed unit ball $B\left(0,1\right)$ and every convex set $C_i$ for all $i \in [r]$, then there exists a $k$-flat $K$ and $j \in [r]$ such that, for all $C \in \F_{j}$, we have
    \begin{equation}
        d(C,K) \leq \sqrt{\frac{1}{r-k}} .
    \end{equation}
\end{theorem}
Observe that by substituting $\F_{1} = \F_{2} = \dots = \F_{r} = \F$ in Theorem~\ref{main-result}
we get the following theorem. 

\begin{theorem}[No-Dimensional Helly Theorem for $k$-flats]
    \label{noDimKflat}
    Let $\F$ be a $k$-unbounded family of convex sets in $\R^d$ and there exists an $R > 0$ such that $\forall C \in \F$ we have have 
    $\diam(C) < R$.
    For $r \in \N$ with $k < r \leq d$ and $b \in \R^{d}$, if for every $C_{1}, C_{2}, \dots,C_r$ in $\F$ there exists a $k$-flat $H$ that intersects $B(0,1)$ and every $C_i$ for all $i\in\{1,2,\dots,r\}$, then there exists a $k$-flat $K$ such that, for all $C \in \F$, we have 
    $$
        d(C,K) \leq \sqrt{\frac{1}{r-k}} \; .
    $$
\end{theorem}

\noindent 
If each $\F_{i}$ in Theorem~\ref{main-result} is $k$-unbounded then we get the following colorful generalization of the above Theorem~\ref{noDimKflat}.

\begin{theorem}[Colorful generalization of Theorem~\ref{noDimKflat}]\label{colorNoDimKflat}
    Let $\F_{1}, \dots, \F_{r}$ be $k$-unbounded families of convex sets in $\R^d$ where $k<r\leq d$, and there exists $R > 0$ such that $\forall C \in \F_{1}\cup \dots \cup \F_{r}$ we have $\diam(C) < R$. 
    If for any $r$-tuple $\left(C_{1}, \dots, C_{r}\right) \in \F_{1}\times \dots \times \F_{r}$ there exists a $k$-flat that intersects the closed unit ball $B\left(0,1\right)$ and every convex set $C_i$ for all $i \in \{1, \dots, r \}$, then there exists a $k$-flat $K$ and $j \in \{1, \dots, r\}$ such that, for all $C \in \F_{j}$, we have
    \begin{equation*}
        d(C,K) \leq \sqrt{\frac{1}{r-k}} \; .
    \end{equation*}
\end{theorem}

In the above theorems we require the convex sets to have bounded diameter. Note that this condition cannot be relaxed. Consider hyperplanes in $\R^{d}$ and observe that any finite collection of hyperplanes can be pierced by a line passing through the origin $\mathcal{O}$ in $\R^{d}$. But, for any $k$-flat $K$, with $k \leq d-1$, and $\forall \Delta > 0$ there exists a hyperplane $H$ such that $d\left( K, H\right) > \Delta$. The following two results will complement our results on no-dimensional Helly Theorem by showing the tightness of the bound guaranteed by our results and also show that the $k$-unboundedness condition is unavoidable. 


\begin{theorem}[On families not being $k$-unbounded]
There exists a family $\cF$ of convex sets in $\R^{3}$ such that 
    \begin{itemize}
        \item 
            there exists $R > 0$ such that $\diam(C) < R$ for all $C \in \cF$,

        \item
            $\cF$ is $1$-unbounded,
            
        \item
            any three convex sets in $\cF$ can be pierced by a plane ($2$-dimensional affine space) passing through the origin $\mathcal{O}$, and
            
        \item
            for any plane $K$ in $\R^{3}$ there exists a $C_{K} \in \cF$ such that $d\left( K, C_{K}\right) > 1$.
    \end{itemize}
\label{impossibility1}
\end{theorem}





\begin{theorem}[Tightness of the bound in Theorem~\ref{main-result}]\label{impossibility2}
There exist families $\cF_{1}, \cF_{2}, \cF_{3}$ of convex sets in $\R^{3}$ satisfying the following properties:
    \begin{itemize}
        \item 
            $\forall C \in \cF_{1} \cup \cF_{2} \cup \cF_{3}$, $\diam(C) = \sqrt{2}$,
                
        \item 
            both $\cF_{1}$ and $\cF_{2}$ are $1$-unbounded,
                
        \item
            $\forall (C_{1}, C_{2}, C_{3}) \in \cF_{1} \times \cF_{2} \times \cF_{3}$ there exists a line $L$ that pierces $C_{1}, C_{2}, C_{3}$, and $d(L, \mathcal{O}) \leq 1$, and
        
        \item
            for every line $K$ in $\R^{3}$ there exists $j \in [3]$ such that 
            $$
                \max\limits_{C \in \cF_{j}} d(C, K) \geq \frac{1}{\sqrt{2}}.
            $$
    \end{itemize}
\end{theorem}



==> proof.tex <==
\section{Proofs of the claimed results}
\label{sec-proof}


In this section we will give the proofs of the results claimed in Section~\ref{defth}. We will first begin by proving the following colorful generalization of the Helly Theorem for $k$-flats proved by Aronov, Goodman and Pollack~\cite{AronovGP2002}.
\begin{theorem}
    [Restatement of Theorem~\ref{col_aronov1}]
    \label{restatement-col_aronov1}
    Suppose for each $i\in[d+1], \cS_i$ is a $k$-unbounded collection of compact convex sets in $\R^{d}$, and there exists $R > 0$ such that $\forall C \in \cS_{i}$ we have $\diam(C) < R$. 
    Also, assume that for every $(d+1)$-tuple $(C_{1}, \dots, C_{d+1}) \in \cS_{1}\times \dots \times \cS_{d+1}$ there exists a $k$-flat $H$ such that $H$ intersects $C_{i}$ for all $i \in [d+1]$. Then $\exists j\in[d+1]$ and a $k$-flat $\widetilde{H}$ that intersects every sets in $\cS_{j}$.
\end{theorem}

\begin{proof}
Suppose for each $i\in[d+1],\; \cL_i$ is a set of $k$ linearly independent vectors in the limiting directions set $LDS(\cS_i)$ of $\cS_i$. Then there exists a linearly independent set of $k$ vectors, say $\cL=\{z_1,\dots, z_k\}$, such that for each $i\in [k],\;z_i\in\cL_i$. Suppose $\cK$ is the $k$-flat generated by the linear span of $\cL$. Now for each $i\in [k]$, since $z_i\in\cL_i$, so $\exists$ a sequence $\{S_{i,n}\}_{n\in\NN}$ in $\cS_i$ and for each $n\in\NN$, $\exists x_{i,n}\in S_{i,n}$ such that $||x_{i,n}||\to\infty$ as $n\to\infty$ and the sequence $\{f(x_{i,n})\}_{n\in\NN}$ converges to $z_i$, as $n\rightarrow\infty$.

Now if $\exists i\in [k]$ such that $\cS_i$ has a $k$-transversal then there is nothing to prove. Otherwise for each $i\in [d+1], i>k$, we take any $B_i\in\cS_i$ and take any $n\in\NN$. Then $B_{k+1},\dots, B_{d+1}$ together with $S_{1,n},\dots, S_{k,n}$, as a colorful tuple, is pierceable by a $k$-flat. This follows that $B_{k+1},\dots, B_{d+1}$ can be pierced by a $k$-flat arbitrarily close to the direction of $\cK$. So by compactness of $B_i$'s we can say that, $B_{k+1},\dots, B_{d+1}$ can be pierced by a $k$-flat in the direction of $\cK$, i.e, parallel to $\cK$.

Now for each $i\in [d+1],\; i>k$, suppose $\cS'_i$ is the projected family of $\cS_i$ on the $(d-k)$ dimensional space $\cK^{\perp}$, orthogonal to $\cK$. Then every colorful $(d-k+1)$ tuple from $\cS'_{k+1},\dots,\cS'_{d+1}$ is pierceable by a point in the space $\cK^{\perp}$. So by \emph{Colorful Helly's Theorem}, $\exists i\in [d+1],\; i>k$ such that $\cS'_i$ is pierceable by a point in $\cK^{\perp}$. Hence there exists a $k$-flat parallel to $\cK$ that hits all the members of the family $\cS_i$.
\end{proof}











\begin{theorem}[Restatement of~\ref{main-result}]
    \label{main-result1}
    Let $\F_{1}, \dots, \F_{r}$ families of convex sets in $\R^{d}$, $k < r \leq d$, and the family $\F:= \F_{1} \cup \dots\cup \F_{r}$ of convex sets satisfy the following properties:
    \begin{enumerate}
        \item[(i)] 
            $\exists R > 0$ such that for all $C \in \F$ we have $\diam(C) < R$

        \item[(ii)]
            $\exists J_{k} = \{ j_{1}, \dots, j_{k}\} \subset [r]$ and $\left\{ y_{j_{1}}, \dots, y_{j_{k}}\right\} \subset \mathbb{S}^{d-1}$ such that 
            \begin{itemize}
                \item 
                    for all $i \in J_{k}$ we have $y_{i} \in LDS\left( \F_{i} \right)$, and 
                \item 
                    the collection of vectors $\left\{ y_{j_{1}}, \dots, y_{j_{k}}\right\}$ are linearly independent 
            \end{itemize}
    \end{enumerate}
    If for any $r$-tuple $\left(C_{1}, \dots, C_{r}\right) \in \F_{1}\times \dots \times \F_{r}$ there exists a $k$-flat that intersects the closed unit ball $B\left(0,1\right)$ and every convex set $C_i$ for all $i \in \{1, \dots, r \}$, then there exists a $k$-flat $K$ and $j \in \{1, \dots, r\}$ such that, for all $C \in \F_{j}$, we have
    \begin{equation*}
        d(C,K) \leq \sqrt{\frac{1}{r-k}} .
    \end{equation*}
\end{theorem}


\begin{proof}
Suppose for any set $F\subset \RR^d$, $\Bar{F}$ is the closure of $F$. Since for any point $p\in\RR^d$, $d(p,F)=d(p,\Bar{F})$, it is enough to show that $\exists j\in [r]$ such that there exists a $k$-flat $K$ satisfying $\forall C \in \F_{j}$, 
        $$d(\Bar{C},K) \leq \sqrt{\frac{1}{r-k}}.$$
        
Now without loss of generality, we assume that $J_k=[k]$. Then for each $j\in J$, $y_j\in\mathrm{LDS}(\cF_j)$ implies that $\exists\text{ a sequence }\{F_{j,n}\}_{n\in\NN}$ in $\cF_j$ and for each $n\in\NN,\;\exists x_{j,n}\in\F_{j,n}$ such that the sequence $\{f(x_{j,n})\}_{n\in\NN}$ converges to $y_j$. 

Now if $\exists j\in [r]$ such that there exists a $k$-flat $K$ satisfying $\forall C \in \F_{j}$, 
        $d(C,K) \leq \sqrt{\frac{1}{r-k}}$, then there is nothing to prove.
Otherwise, suppose $K$ is the $k$-flat generated by the linear span of $\{y_1,\dots,y_k\}$. Now for each $i\in [r],\; i>k,$ take any $F_i\in\cF_i$. Then for each $n\in\NN$, there exists a $k$-flat $K_n$ intersecting $B(0,1)$ and piercing $F_{1,n},F_{2,n},\dots, F_{k,n}, F_{k+1},\dots, F_r$. This implies that $F_{k+1},\dots, F_r$ can be pierced by a $k$-flat arbitrarily close to the direction of $K$. 
Now by compactness of $\Bar{F_i}$'s, we conclude that $\exists a\in K^{\perp}$ such that the $k$-flat $a+K$ pierces $\Bar{F}_{k+1},\dots,\Bar{F}_r$.
Since $a+K$ intersects $B(O,1)$, we must have $\|a\|\leq 1$.

Now let for any set $A$ in $\R^d$, $\pi(A)$ denote the orthogonal projection of $A$ onto the $(d-k)$-dimensional space $K^{\perp}$. Then for any $(C_{k+1},\dots C_r)\in\cF_{k+1}\times\dots\times\cF_r$, we have 
$$
    \left(\bigcap_{i=k+1}^r \pi\left(\Bar{C_i}\right) \right)\bigcap B(0,1)\neq\emptyset.
$$
Then, by Theorem~\ref{PointColor}, $\exists q\in K^{\perp}$ and $\exists i\in\{k+1,\dots, r\}$ such that $\forall C\in\cF_i$ we have
$$
    d \left( q, \pi \left( \overline{C} \right) \right)<\sqrt{\frac{1}{r-k}} \; .
$$ 

Suppose $q'\in \pi^{-1}(q)$ and consider the $k$-flat $K'=q'+K$. Then we have $\forall C\in\cF_i$, $$
    d\left( K',\overline{C} \right) <\sqrt{\frac{1}{r-k}} \; .
$$ 
\end{proof}



















%\begin{theorem}[Restatement of Theorem~\ref{noDimKflat}]
%    \label{restatement-noDimKflat}
%    Let $\F$ be a $k$-unbounded family of compact convex sets in $\R^d$ and there exists an $R > 0$ such that $\forall C \in \F$ we have have 
%    $\diam(C) < R$.
%    For $r \in \N$ with $k < r \leq d$ and $b \in \R^{d}$, if for every $C_{1}, C_{2}, \dots,C_r$ in $\F$ there exists a $k$-flat $H$ such that $H$ intersects $C_i$ for all $i\in\{1,2,\dots,r\}$ and $d (H,b) \leq 1$, then there exists a $k$-flat $K$ such that, for all $C \in \F$, we have
%    \begin{equation}
%        d(C,K) \leq \sqrt{\frac{1}{r-k}} .
%    \end{equation}
%\end{theorem}
%
%\begin{proof}
%    Without loss of generality, let us set the center $b$ of the Euclidian ball, referred to in the theorem, at the origin $O$.
%    For any $S\in\F$ \red{(Will it be $C$ as mentioned in the statement of the theorem???)}, pick a point $s\in S$ and project it onto the unit sphere $\Sigma$ centered at $O$ by the central projection map $f:\R^d\setminus\{O\}\to\Sigma$. Let $\text{LDS}(\F)$ denote the limiting direction set of $\F$ and let $y_1, y_2,\dots, y_k$ be $k$ independent vectors in $\text{LDS}(\F)$. Let $K$ denote the $k$-flat which is the linear span of $y_1,y_2,\dots,y_k$ and let $K^{\perp}$ denote the $(d-k)$-dimensional space orthogonal to $K$. Then there exist $k$ infinite sequence in $\F$, viz, $S_{i,1},S_{i,2},S_{i,3},\dots$, $i \in [N]$, such that the sequence $f(s_{i,1}),f(s_{i,2}),f(s_{i,3}),\dots$ converges to $y_i$, where $s_{i,n}\in S_{i,n}$ $\forall i \in [N]$. Next, we pick any $r-k$ sets $T_1,T_2,\dots,T_{r-k}$ from $\F$. Now, for a given $n\in\mathbb{N}$, there is a $k$-flat that intersects $T_1,\dots,T_{r-k}$,$S_{1,n},\dots,S_{k,n}$ as well as the closed Euclidian ball $\overline{B}(0,1)$ \red{(by the statement of the theorem)}. This means, there exists a $k$-flat that intersects	$T_1,\dots,T_{r-k}$ and is arbitrarily close to the $k$-flat $K$. In other words, for any $\epsilon>0$, we can find a $k$-flat $a_{\epsilon}+K_{\epsilon}$ that intersects $T_1,\dots,T_{r-k}$,$S_{1,n},\dots,S_{k,n}$ as well as $\overline{B}(0,1)$, where $K_{\epsilon}$ is a $k$-dimensional linear subspace of $\R^d$, such that $\forall x\in K_{\epsilon}\cap \Sigma$ there is a $y\in K\cap\Sigma$ with $d(x,y)<\epsilon$. We take $a_{\epsilon}$ to be in $K^{\perp}$. Now, as $a_{\epsilon}+K_{\epsilon}$ intersects $\overline{B}(0,1)$, we have $a_{\epsilon}\in \overline{B}(0,1)$. Since each $T_j$ is compact, $j\in[r-k]$, there must exist a $k$-flat $a+K$ that intersects each $T_j$, where $a$ is in $\overline{B}(0,1)\cap K^{\perp}$. Let us now project $\R^d$ onto $K^{\perp}$. The projections of $T_1,\dots,T_{r-k}$ onto $K^{\perp}$ intersect at $a$, which lie in the unit ball in $K^{\perp}$. Now we can apply Theorem \ref{Point} to obtain a $q\in K^{\perp}$ such that if $T'$ is the projection of $T\in\F$ onto $K^{\perp}$, then $d(q,T')\leq \sqrt{\frac{1}{r-k}}$ $\forall T\in\F$, and therefore, $q+K$ is the $k$-flat that satisfies the property stated in Theorem \ref{noDimKflat}.
%\end{proof}
%
%
%\begin{theorem}[Restatement of Theorem~\ref{colorNoDimKflat}]\label{restatement-colorNoDimKflat}
%    Let $\F_{1}, \dots, \F_{r}$ be $k$-unbounded families of compact convex sets in $\R^d$ where $k<r\leq d$, and $b \in \R^{d}$. 
%    If for any $r$-tuple $\left(C_{1}, \dots, C_{r}\right) \in \F_{1}\times \dots \times \F_{r}$ there exists a $k$-flat that intersects the closed unit ball $B\left(0,1\right)$ and every convex set $C_i$ for all $i \in \{1, \dots, r \}$, then there exists a $k$-flat $K$ and $j \in \{1, \dots, r\}$ such that, for all $C \in \F_{j}$, we have
%    \begin{equation}
%        d(C,K) \leq \sqrt{\frac{1}{r-k}} .
%    \end{equation}
%    
%    \textcolor{red}{
%    In fact, the condition that each $\F_i$ has to be $k$-unbounded can be replaced with the weaker condition that $\F\coloneqq\cup_{i\in[r]}\F_i$ is $k$-unbounded, and we can find a subset $\{j_1,j_2,\dots,j_k\}\subset[r]$ of size $k$ such that for each $i\in\{j_1,j_2,\dots,j_k\}$, $\F_i$ is at least $1$-unbounded, and there exist $k$ independent vectors $y_{j_1},y_{j_2},\dots,y_{j_k}$ such that there are unbounded sequences $S_{i,1},S_{i,2},\dots,S_{i,n},\dots$ in $\F_i$ for $i\in\{j_1,j_2,\dots,j_k\}$ such that $S_{i,n}\in\F_i$ for all $i\in\{j_1,j_2,\dots,j_k\}\subset[r]$ and $n\in\N$, and for $s_{i,n}\in S_{i,n}$, $f(s_{i,n})\to y_i$ as $n\to\infty$.
%    }
%\end{theorem}
%
%
%
%
%\begin{proof}
%    In fact, the condition that each $\F_i$ has to be $k$-unbounded can be replaced with the weaker condition that $\F\coloneqq\cup_{i\in[r]}\F_i$ is $k$-unbounded, and we can find a subset $\{j_1,j_2,\dots,j_k\}\subset[r]$ of size $k$ such that for each $i\in\{j_1,j_2,\dots,j_k\}$, $\F_i$ is at least $1$-unbounded, and there exist $k$ independent vectors $y_{j_1},y_{j_2},\dots,y_{j_k}$ such that there are sequences $S_{i,1},S_{i,2},\dots,S_{i,n},\dots$ in $\F_i$ for $i\in\{j_1,j_2,\dots,j_k\}$ such that $S_{i,n}\in\F_i$ for all $i\in\{j_1,j_2,\dots,j_k\}\subset[r]$ and for $s_{i,n}\in S_{i,n}$, $f(s_{i,n})\to y_i$ as $n\to\infty$.
%	Let $K$ denote the $k$-dimensional linear subspace generated by $y_{j_1},y_{j_2},\dots,y_{j_k}$. 
%	Pick any $r-k$ sets $T_{i_1},T_{i_2},\dots,T_{i_{r-k}}$ where $T_{i_j}\in\F_{i_j}$, $i_j\in[r]\setminus\{j_1,j_2,\dots,j_k\}$. Similar arguments as in the proof of Theorem \ref{noDimKflat} show that there exists a $k$-flat $a+K$ that intersects $T_{i_1},T_{i_2},\dots,T_{i_{r-k}}$ as well as $\overline{B}(0,1)$ where $a\in \overline{B}(0,1)\cap K^{\perp}$.
%	Now as before, we project $\R^d$ onto $K^{\perp}$ and apply Theorem \ref{PointColor}, which gives us the conclusion in Theorem~\ref{colorNoDimKflat}.
%\end{proof}


\begin{theorem}[On families not being $k$-unbounded: Restatement of Theorem~\ref{impossibility1}]
There exists a family $\cF$ of convex sets in $\R^{3}$ such that
    \begin{itemize}
        \item 
            there exists $R > 0$ such that $\diam(C) < R$ for all $C \in \cF$,

        \item
            $\cF$ is $1$-unbounded,
                
        \item
            any three convex sets in $\cF$ can be pierced by a plane ($2$-dimensional affine space) passing through the origin $\mathcal{O}$, and
            
        \item
            for any plane $K$ in $\R^{3}$ there exists a $C_{K} \in \cF$ such that $d\left( K, C_{K}\right) > 1$.
    \end{itemize}
\label{restatement-impossibility1}
\end{theorem}


%\begin{figure}
%    \centering
%    \includegraphics[scale = 0.80]{old_version/newfigure1.pdf}
%    \caption{}
%    \label{fig-convex-set-being-bounded}
%\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale = 1.20]{kUGimp.pdf}
    \quad\quad
    \includegraphics[width = 5.0cm, height= 5.0cm]
    {newfigure-3.pdf}
    \caption{An example demonstrating the necessity of $k$-unboundedness condition. This figure has been taken from~\cite{AronovGP2002}.}
    \label{fig:k1}
\end{figure}
\begin{proof}
To establish the necessity of $k$-unboundedness we will be using a construction that is closely related to the one given by Aronov et al.~\cite{AronovGP2002}. 

            
            Consider the eight shaded convex regions in Figure~\ref{fig:k1} created by four circles and four squares centered at a point $\mathcal{O}$. Let $x_{3} = 0$ be the plane that contains the Figure~\ref{fig:k1}, and without loss of generality assume that $\mathcal{O}$ be the origin in $\R^{3}$. We will call these eight shaded convex regions $a_1$, $a_2$, $\dots$, $a_8$, respectively. Observe that any $3$ of these convex sets can be intersected by a straight line passing $\mathcal{O}$. 
            
            We will now create additional convex sets in the following way: we choose the eight convex sets in a fixed order, and in each step elevate the sets in increasing heights in that order along the $x_{3}$-axis such that for any $n\in\N$ there are infinitely many sets of this collection that lie outside $B\left(\mathcal{O},n\right)$. This gives us a countably infinite sequence $\F$ of sets, where $\F$ is $1$-unbounded, but not $2$-unbounded.
            Clearly, for any three sets in $\F$, there exists a plane that passes through $\mathcal{O}$ and intersects these sets. 
    
    Let $\ell$ denote the length of the side of the smallest square in Figure \ref{fig:k1}.
    We show that it is not possible to find a plane that is at most a distance 1 unit away from all the sets in $\F$ when $\ell$ is large enough.
    Let $K$ be a plane for which the maximum distance from the sets in $\F$ is minimized, and $l_{K}$ be the intersection of $K$ with the plane $x_{3} = 0$. Clearly, $K$ must be perpendicular to the plane that contains the first $8$ sets, because otherwise for any $R>0$ we would find a set $C$ in $\F$ for which $d(K,C)>R$.
    Consider the straight line $l_{K}$ that is the intersection of $K$ and the plane given by the equation $x_{3} = 0$.
    If $l_{K}$ is moved on the $x_{3} = 0$ plane closer to $\mathcal{O}$ along the line perpendicular to $l_{K}$ from $\mathcal{O}$, the quantity $\max\left\{d\left(a_{2n},l_{K}\right),d\left(a_{2n-1},l_{K}\right)\right\}$ does not increase for $n \in \left\{ 1,2,3,4 \right\}$.
    Since $d(K,a_i)=d(l_{K},a_i)$ $\forall i\in[8]$, we can take $K$ to be passing through $\mathcal{O}$. Let the side-lengths of the $4$ squares in Figure \ref{fig:k1} be $\ell_{1}\, (=\ell), \ell_{3}, \ell_{5}, \ell_{7}$, where the side of side-length $\ell_{i}$ is shared by the set $a_{i}$.
    Let the diagonals of the largest square in Figure \ref{fig:k1} lie on the $x_{1}$-axis and the $x_{2}$-axis respectively.
    Then, if $l_{K}$ makes an angle $\theta\in[0,\pi)$ with the $x_{1}$-axis, then we have the following: for $i \in \left\{ 1, 3, 5, 7 \right\}$ we have 
    \begin{align}
        d\left(a_{i}, l_{K} \right) = d \left( a_{i+1}, l_{k} \right),
    \end{align}
    and
    \begin{align}
        d(a_{1},l_{K}) &=
                \begin{cases}
                    \frac{\ell_1}{\sqrt{2}}\sin\left({\pi}/{4}-\theta \right) & \text{if } 0\leq\theta\leq {\pi}/{4}\\
                    \frac{\ell_1}{\sqrt{2}} \sin\left(\pi-\theta\right) & \text{if } {3\pi}/{4} \leq \theta \leq \pi \\
                    0 & \text{otherwise}
                \end{cases} \\
        d(a_{3},l_{K}) &=
                \begin{cases}
                    \frac{\ell_3}{\sqrt{2}}\sin\theta & \text{if } 0 \leq \theta \leq {\pi}/{4} \\
                    \frac{\ell_3}{\sqrt{2}}\sin\left({\pi}/{2}-\theta\right) & \text{if } {\pi}/{4} \leq \theta \leq {\pi}/{2} \\
                    0 & \text{otherwise}
                \end{cases} \\
        d(a_{5},l_{K}) &=
                \begin{cases}
                    \frac{\ell_5}{\sqrt{2}}\sin\left(\theta - {\pi}/{4}\right) & \text{if } {\pi}/{4} \leq \theta \leq {\pi}/{2}\\
                    \frac{\ell_5}{\sqrt{2}}\sin \left( {3\pi}/{4}-\theta \right) & \text{if }{\pi}/{2} \leq \theta \leq {3\pi}/{4}\\
                    0 & \text{otherwise}
                \end{cases} \\
        d(a_7,l_{K}) &=
                \begin{cases}
                    \frac{\ell_7}{\sqrt{2}}\sin\left(\theta - {\pi}/{2}\right) & \text{if }{\pi}/{2} \leq \theta \leq {3\pi}/{4} \\
                    \frac{\ell_7}{\sqrt{2}} \sin \left(\pi-\theta\right) & \text{if } {3\pi}/{4} \leq \theta \leq \pi \\
                    0 & \text{otherwise}
                \end{cases}
    \end{align}
    Now, observe that 
    \begin{align*}
        \sum_{i=1}^{8} d\left(a_{i},l_{K}\right) &\geq \frac{\ell}{\sqrt{2}} \times 
        \min_{\theta\in \left[0, {\pi}/{4}\right]} \left(\sin\theta + \sin\left({\pi}/{4}-\theta \right)\right) \\
        &\geq \ell\sqrt{2}\sin\left({\pi}/{8}\right)
    \end{align*}
    Thus, for $\ell>\sqrt{2}/\sin\left({\pi}/{8}\right)$, there are no planes that are at most $1$ distance away from each set in $\F$.
\end{proof}



\begin{theorem}[Tightness of the bound in Theorem~\ref{main-result}: Restatement of Theorem~\ref{impossibility2}]\label{restatement-impossibility2}
There exist families $\cF_{1}, \cF_{2}, \cF_{3}$ of convex sets in $\R^{3}$ satisfying the following properties:
    \begin{itemize}
        \item 
            $\forall C \in \cF_{1} \cup \cF_{2} \cup \cF_{3}$, $\diam(C) = \sqrt{2}$,
                
        \item 
            both $\cF_{1}$ and $\cF_{2}$ are $1$-unbounded,
                
        \item
            $\forall (C_{1}, C_{2}, C_{3}) \in \cF_{1} \times \cF_{2} \times \cF_{3}$ there exists a line $L$ that pierces $C_{1}, C_{2}, C_{3}$, and $d(L, \mathcal{O}) \leq 1$ and
        
        \item
            for every line $K$ in $\R^{3}$ there exists $j \in [3]$ such that 
            $\max\limits_{C \in \cF_{j}} d(C, K) \geq \frac{1}{\sqrt{2}}$.
    \end{itemize}
\end{theorem}





\begin{proof}
We provide an example where the bound given in Theorem~\ref{colorNoDimKflat} is tight.
    


\begin{figure}
\centering
\includegraphics[width = 5.0cm, height = 9.50cm]{newfigure-2.pdf}
\caption{An example demonstrating the tightness of the bound given in Theorem~\ref{impossibility2}.}
\label{fig:bound2}
\end{figure}







    
Let $\{A,B,C,D,E,F,G,H\}$ be the $8$ vertices cube in $\R^3$ whose centroid is the origin $\cO$ and side length is $\sqrt{2}$ and $EFGH$ is parallel to the plane $x_3=0$ (see Figure~\ref{fig:bound2}).
Define $\F_i\coloneqq\{S_{i,1},S_{i,2},S_{i,3},\dots\}$ for $i=1,2,3$ in the following way: Set $S_{1,1}=\ol{AB}$, $S_{1,2}=\ol{CD}$ and for $n>2$, $S_{1,n}$ is the line segment $\ol{CD}$ raised to the height $x_3=n$. Similarly, set $S_{2,1}=\ol{GH}$, $S_{1,2}=\ol{EF}$ and for $n>2$, $S_{2,n}$ is the line segment $\ol{EF}$ lowered to the height $x_3=-n$. Now set $S_{3,1}=\ol{BC},S_{3,2}=\ol{DA},S_{3,3}=\ol{FG},S_{3,4}=\ol{HE}$, and let $S_{3,4n+j}$ be the set $S_{3,j}$, for all $j \in \{0,1,2,3\}$ (see Figure~\ref{fig:bound2}). Clearly, any colorful $3$-tuple $(C_1,C_2,C_3)$, $C_i\in\F_i$, $i\in[3]$, can be hit by a straight line that is at most at a distance $1$ away from the centroid. Let $\mathcal{L}$ denote the set of all straight line transversals $l$ of colorful $3$-tuples such that $l$ is as close to $\cO$ as possible. Let $l_n$ denote the straight line transversal in $\mathcal{L}$ that passes through $S_{1,n},S_{2,1},S_{3,1}$. Clearly, $d(l_n,\cO)\to 1$ as $n\to\infty$.
Then $$\sup_{l\in\mathcal{L}}d(\cO,l)=1.$$
Now note that for the straight line $L$ that is perpendicular to the plane on which $ABCD$ lies and passes through $\cO$, we have $$\inf_{i\in[3]}\sup_{C\in\F_i}d(l,C)\ge\inf_{i\in[3]}\sup_{C\in\F_i}d(L,C),$$ for any straight line $l$ in $\R^3$. This we can show in the following way: let $l_1$ be a straight line such that $$\sup_{C\in\F_1}d(l_1,C)=\inf_{l\in\mathcal{L}}\sup_{C\in\F_1}d(C,l).$$
Then $l_1$ must be perpendicular to the plane on which $ABCD$ lies, otherwise, the supremum of its distances from sets in $\F_1$ would be infinity. Then, $l_1$ must be equidistant from both $S_{1,1}$ and $S_{1,2}$, and therefore, we can take $l_1$ to be $L$. Similar arguments show that 
$$
    \sup_{C\in\F_2}d(L,C)=\inf_{l\in\mathcal{L}}\sup_{C\in\F_1}d(C,l).
$$ 
We have $$\inf_{i\in[3]}\sup_{C\in\F_i}d(L,C)=\frac{1}{\sqrt{2}}.$$
To see that $$\inf_{l\in\mathcal{L}}\sup_{C\in\F_3}d(C,l)=\frac{1}{\sqrt{2}},$$ project $\ol{BC}$, $\ol{AD}$, $\ol{FG}$, $\ol{EH}$ onto the plane $P$ that contains $ABEF$. If there is a straight line $l_3$ such that 
$$
    \sup_{C\in\F_3}d(l_3,C)=\inf_{l\in\mathcal{L}}
    \sup_{C\in\F_3}d(C,l),
$$ 
then let the projection of $l_3$ onto $P$ be $l'_3$. If $L$ is not the straight line that minimizes $$\inf_{l\in\mathcal{L}}\sup_{C\in\F_6}d(C,l),$$ then the perpendicular distance from $l'_3$ to $A,B,E$ and $F$ must be smaller than $\frac{1}{\sqrt{2}}$. Let, without loss of generality, $A$ be the point from which $l'_3$ is the farthest. Then, we must have another point among $B,E,$ and $F$ from which $l'_3$ has the same distance as $A$. This point then must be $E$, because otherwise, we could have taken $L$ to be $l_3$. This means that $l'_3$ passes through the centroid of the square $ABEF$ and two points from $A,B,E,$ and $F$ lie on each side of $l'_3$. But this implies that $l'_3$ must be parallel to $AB$ since $l'_3$ has the minimum distance from both $A$ and $B$ and is at least as close to $E$ and $F$, which is a contradiction. We have $$\inf_{i\in[3]}\sup_{C\in\F_i}d(L,C)=\frac{1}{\sqrt{2}},$$ which is what we get by plugging in the values of $r$ and $k$ in the inequality given in Theorem~\ref{colorNoDimKflat}.
\end{proof}




















